Quantum Computing from Graphs

While stabilizer tableaus have proven exceptionally useful as a descriptive tool for additive quantum codes, they offer little guidance for concrete constructions or coding algorithm analysis. We introduce a representation of stabilizer codes as graphs with certain structures. Specifically, the graphs take a semi-bipartite form where input nodes map to output nodes, such that output nodes may connect to each other but input nodes may not. Intuitively, the graph's input-output edges represent information propagation of the encoder, while output-output edges represent the code's entanglement. We prove that this graph representation is in bijection with tableaus and give an efficient compilation algorithm that transforms tableaus into graphs. We show that this map is efficiently invertible, which gives a universal recipe for code construction by finding graphs with nice properties. The graph representation gives insight into both code construction and algorithms. To the former, we argue that graphs provide a flexible platform for building codes. We construct several constant-size codes and several infinite code families. We also use graphs to extend the quantum Gilbert-Varshamov bound to a three-way distance-rate-weight trade-off. To the latter, we show that key coding algorithms, distance approximation, weight reduction, and decoding, are unified as instances of a single optimization game on a graph. Moreover, key code properties such as distance, weight, and encoding circuit depth, are all controlled by the graph degree. We give efficient algorithms for producing encoding circuits whose depths scale with the degree and for implementing certain logical diagonal and Clifford gates with reduced depth. Finally, we find an efficient decoding algorithm for certain classes of graphs. These results give evidence that graphs are useful for the study of quantum computing and its implementations.

==> fontsets/mitthesis-defaultfonts.tex <==
% From mitthesis package
% Documentation: https://ctan.org/pkg/mitthesis

\ProvidesFile{mitthesis-defaultfonts.tex}[2024/09/14 v1.05 Load Computer/Latin Modern text and math fonts]

%% Default fonts
\ifpdftex
	\ClassNoteNoLine{\ClassName}{Loading Computer Modern text and math fonts (default for pdftex)}
	\RequirePackage[T1]{fontenc} % With T1 encoding, pdftex will silently load the cm-super fontset
%   \RequirePackage[]{babel} % load babel (with desired options) if using a language other than English
	\RequirePackage{bm}
\else
	\ClassNoteNoLine{\ClassName}{Loading Latin Modern text and math fonts (default for unicode engines)}
	%
%   \RequirePackage[]{babel} % load babel (with desired options) if using a language other than English
    \RequirePackage[warnings-off={mathtools-colon,mathtools-overbracket}]{unicode-math}
    % suppress tiresome warnings about lack of integration between mathtools and unicode-math.
    % Unicode-math loads fontspec package, but default fonts are not selected by fontspec in this case.
\fi


==> fontsets/mitthesis-fira-newtxsf.tex <==
% From mitthesis package
% Documentation: https://ctan.org/pkg/mitthesis

\ProvidesFile{mitthesis-fira-newtxsf.tex}[2024/10/10 v1.06 Load Fira Sans text font with newtx sans serif math font and Inconsolata typewriter font]

%% Adjusted sizes of text, math, and typewriter fonts, 2024/10/11
%% Fira Sans text font with newtx sans serif math font and Inconsolata typewriter font
%
\ifpdftex
	\ClassNoteNoLine{\ClassName}{Loading Fira sans text font with newtx sans serif math font and Inconsolata typewriter}
	\RequirePackage[U,T1]{fontenc}
    \RequirePackage[varqu,varl]{zi4} % inconsolata font for typewriter
    \RequirePackage[sfdefault,tabular,lf]{FiraSans} % sans serif text package
    % Use option lf to get lining figures rather than default, old style figures. Use tabular to get tabular figures, not proportional figures.
    % Best choice will vary, depending on what type of content you have. With some effort, these settings can be changed according to content,
    % See, e.g.: https://tex.stackexchange.com/q/114331/119566
    \renewcommand\rmdefault{\fira@family} % roman font for math (e.g., for operators) and for \textrm{..}
    \RequirePackage[scaled=1.1]{newtxsf}  % sans serif math; [noSTIXops] option suppresses STIX figures in favor of text font figures, 
    % in the most recent versions of newtxsf, but using the following for backward compatibility. NB: 'figures' means numbers: 0123456789.
    % This matters, for example, in tables that mix text and math figures.
        \DeclareSymbolFont{mynumbers}{T1}{FiraSans-TLF}{m}{n}
        \DeclareMathSymbol{0}{\mathord}{mynumbers}{`0}
        \DeclareMathSymbol{1}{\mathord}{mynumbers}{`1}
        \DeclareMathSymbol{2}{\mathord}{mynumbers}{`2}
        \DeclareMathSymbol{3}{\mathord}{mynumbers}{`3}
        \DeclareMathSymbol{4}{\mathord}{mynumbers}{`4}
        \DeclareMathSymbol{5}{\mathord}{mynumbers}{`5}
        \DeclareMathSymbol{6}{\mathord}{mynumbers}{`6}
        \DeclareMathSymbol{7}{\mathord}{mynumbers}{`7}
        \DeclareMathSymbol{8}{\mathord}{mynumbers}{`8}
        \DeclareMathSymbol{9}{\mathord}{mynumbers}{`9}
 	\RequirePackage{bm}
\else
	\ClassWarning{\ClassName}{The fira-newtxsf font set requires pdflatex. Defaulting to LMR fonts}
    \RequirePackage[warnings-off={mathtools-colon,mathtools-overbracket}]{unicode-math}
    % suppress tiresome warnings about lack of integration between mathtools and unicode-math.
    % Unicode-math loads the fontspec package, but the default fonts are not selected by fontspec in this case.
\fi


==> fontsets/mitthesis-heros-stix2.tex <==
% From mitthesis package
% Documentation: https://ctan.org/pkg/mitthesis

\ProvidesFile{mitthesis-heros-stix2.tex}[2024/10/13 v1.05 Load TeX Gyre Heros (sans serif) text font with STIX Two Math font and Inconsolata monospaced font]

%% TeX Gyre Heros (sans serif) text font with STIX Two Math font and Inconsolata monospaced font
%
% These fonts are available at: 
%				http://www.gust.org.pl/projects/e-foundry/tex-gyre 
%				https://github.com/stipub/stixfonts 
%				https://ctan.org/tex-archive/fonts/inconsolata
% Install these as system fonts on your computer
%
\ifpdftex
	\ClassError{\ClassName}{The heros-stix2 fontset requires a unicode engine. Defaulting to CMR fonts}{To use the class option [fontset=heros-stix2] you must use a unicode engine, such as LuaLaTeX.}
	\RequirePackage[T1]{fontenc}
	\RequirePackage{bm}
\else
	\ClassNoteNoLine{\ClassName}{TeX Gyre Heros (sans serif) text font with STIX2 math font and Inconsolata monospaced font}
	%
    \RequirePackage[warnings-off={mathtools-colon,mathtools-overbracket}]{unicode-math}
    % suppress tiresome warnings about lack of integration between mathtools and unicode-math
    % unicode-math loads the fontspec package

    \setmainfont{texgyreheros}[% Presumes these are system fonts! Available at: http://www.gust.org.pl/projects/e-foundry/tex-gyre
		WordSpace = {1,1.4,1},
		Extension = .otf,
    	UprightFont = *-regular,
    	ItalicFont = *-italic,
    	BoldFont = *-bold,
    	BoldItalicFont = *-bolditalic,
		Numbers = Lining,
    	Scale=0.91,
	]        
    \setsansfont{texgyreheros}[% Presumes these are system fonts! Available at: http://www.gust.org.pl/projects/e-foundry/tex-gyre
		WordSpace = {1,1.4,1},
		Extension = .otf,
    	UprightFont = *-regular,
    	ItalicFont = *-italic,
    	BoldFont = *-bold,
    	BoldItalicFont = *-bolditalic,
		Numbers = Lining,
    	Scale=0.91,
	]        
   \setmonofont{Inconsolatazi4}[% This otf font ships with the LaTeX Inconsolata package and is in CTAN https://ctan.org/tex-archive/fonts/inconsolata
        Scale=1.04,
        Extension = .otf,
        UprightFont = *-Regular,
        ItalicFont = *-Regular,% has no italic face
        BoldFont = *-Bold, 
    	BoldItalicFont = *-Bold,% has no bold italic face
        RawFeature = {+ss01,+ss02,+ss03},
    ]             
    \setmathfont{STIXTwoMath-Regular}[% nice glyphs, but \mkern sometimes needed %% https://github.com/stipub/stixfonts
    	Scale=0.95,%MatchUppercase,%MatchLowercase,
		% scaling is a matter of taste ... the x-heights of STIX2 are greater than for Heros...
    	Extension = .otf,
%		BoldFont = *,% STIX Two Math has no bold face
%       Color=NavyBlue, 
    	RawFeature = {+ss01, -ss02, -ss08},
    ]
    % ss01 -- switch calligraphic to script; +ss02 -- variants of g, u, v, w, z; +ss08 -- upright integrals
    %    
    \setmathfontface\mathbf{STIXTwoText-Bold.otf}[]% to not get Heros bold, https://github.com/stipub/stixfonts
    \setmathfontface\mathit{STIXTwoText-Italic.otf}[]
    \setmathfontface\mathrm{STIXTwoText-Regular.otf}[]% to get roman letters from STIX Two
     %         
    \newcommand*{\FRAC}[1]{{\addfontfeature{Fractions=On}#1}}% use OpenType feature for fractions, \FRAC{1/2} 
\fi


==> fontsets/mitthesis-libertinus.tex <==
% From mitthesis package
% Documentation: https://ctan.org/pkg/mitthesis

\ProvidesFile{mitthesis-libertinus.tex}[2024/10/26 v1.00 Load Libertinus and related fonts]

%% Linux Libertine (serif) text font with newtxmath[libertine] (pdftex) or Libertinus (unicode) math font
%
%  These fonts are available here https://ctan.org/tex-archive/fonts/libertine/opentype 
%						 and here https://github.com/alerque/libertinus
% install these as system fonts on your computer
%
\ifpdftex
	\ClassNoteNoLine{\ClassName}{Loading Libertinus type1 text fonts and newtx-libertinus math fonts}
    \RequirePackage[T1]{fontenc}
    \RequirePackage[lf,t,semibold,ScaleTT=0.9]{libertinus} % tabular lining figures
    \RequirePackage[libertinus,vvarbb,subscriptcorrection]{newtxmath}% see package documentation for options
    \RequirePackage{bm}% load after all math to give access to bold math
\else
	\ClassNoteNoLine{\ClassName}{Loading Libertinus OTF text and math fonts}
	%
    \RequirePackage[warnings-off={mathtools-colon,mathtools-overbracket}]{unicode-math}
    % suppress tiresome warnings about lack of integration between mathtools and unicode-math
    % unicode math loads the fontspec package
 	%
    \setmainfont{LibertinusSerif}[% 
    	Extension = .otf,
    	UprightFont = *-Regular,
    	ItalicFont = *-Italic,
    	BoldFont = *-Semibold, 
    	BoldItalicFont = *-SemiboldItalic,
    	RawFeature={+ss05,+dlig,+tnum}, 
		% +ss02 would change J, K, R; +ss05 changes W; onum = oldstyle figures; hlig = historical ligatures
        ]    
    \setsansfont{LibertinusSans}[% 
    	Extension = .otf,
    	UprightFont = *-Regular,
    	ItalicFont = *-Italic,
    	BoldFont = *-Bold,
	    BoldItalicFont = *-Bold,% does not have bold italic
    	Scale=MatchUppercase]
	%
    \setmonofont{LibertinusMono}[% 
    	Scale=0.9,% 2024/10/13
	    Extension = .otf,
    	UprightFont = *-Regular,
    	ItalicFont = *-Regular,% does not have italic
    	BoldFont = *-Regular,% does not have bold 
	    BoldItalicFont = *-Regular,% does not have bold italic
	] 
	% 
	\newfontfamily\LibertinusDisplay{LibertinusSerifDisplay-Regular.otf}% a display font, as for titles
	%
	\newfontfamily\LibertinusInitials{LibertinusSerifInitials-Regular.otf}% Large initial letters, as for first word in chapter
	%	     	
    %% a Libertinus math font
    \setmathfont{libertinusmath-regular}[%
     	Extension = .otf,   
    	Scale=MatchUppercase,
%		BoldFont = *,% This font lacks a bold version
    	RawFeature={+ss08},% +ss08 gives slanted integrals (no other features) 	
    	]
	\setmathfont{Latin Modern Math}[range=\nabla,Scale=0.91] % I hate the backward nabla in Libertinus Math...
	
    \newcommand*{\FRAC}[1]{{\addfontfeature{Fractions=On}#1}}% use OpenType feature for fractions, \FRAC{1/2} 
\fi


==> fontsets/mitthesis-lmodern.tex <==
% From mitthesis package
% Documentation: https://ctan.org/pkg/mitthesis

\ProvidesFile{mitthesis-lmodern.tex}[2024/10/23 v1.00 Load Latin Modern text and math fonts]

%% Default fonts
\ifpdftex
	\ClassNoteNoLine{\ClassName}{Loading Latin Modern text and math fonts}
	\RequirePackage[T1]{fontenc}
%   \RequirePackage[]{babel} % load babel (with desired options) if using a language other than English
	\RequirePackage{lmodern}
	\RequirePackage{bm}
\else
	\ClassNoteNoLine{\ClassName}{Loading Latin Modern text and math fonts (default for unicode engines)}
	%
%   \RequirePackage[]{babel} % load babel (with desired options) if using a language other than English
    \RequirePackage[warnings-off={mathtools-colon,mathtools-overbracket}]{unicode-math}
    % suppress tiresome warnings about lack of integration between mathtools and unicode-math.
    % Unicode-math loads fontspec package, but default fonts are not selected by fontspec in this case.
\fi


==> fontsets/mitthesis-lucida.tex <==
% From mitthesis package
% Documentation: https://ctan.org/pkg/mitthesis

\ProvidesFile{mitthesis-lucida.tex}[2024/10/13 v1.04 Load Lucida fonts]

%% Lucida Bright and Lucida Bright Math fonts (available from the TeX Users Group)

\ClassNoteNoLine{\ClassName}{Lucida Bright and Lucida Bright Math fonts}

\ifpdftex
	\RequirePackage[LY1]{fontenc}
	\RequirePackage[expert,vargreek,altbullet]{lucidabr}   % switch text and math fonts 
	% some other options: seriftt (much larger quad size!), lucidasmallscale % 2024/10/13
	\RequirePackage{bm}
\else
    \RequirePackage[warnings-off={mathtools-colon,mathtools-overbracket}]{unicode-math}
    % suppress tiresome warnings about lack of integration between mathtools and unicode-math
    % unicode-math loads the fontspec package

    % FEATURE 	DESCRIPTION 											DEFAULT
    % dlig 		discretionary ligatures (f-ligatures in typewriter fnt) off
    % liga 		standard ligatures (f-ligatures, not monospaced fonts) 	on
    % onum 		old style numbers (Lucida Bright only)					off
    % smcp 		small caps 	(Lucida Bright, upright only)				off
    % zero 		slashed zero (sans and monospaced fonts)				off
    % locl 		script/language specific (localized) forms 				on
    %
    % FEATURE 	FONT 						DESCRIPTION
    % ss01 		Lucida Sans & Typewriter 	use dotted zero: 𝟶 vs. default 0.
    % ss01 		use Lucida-standard shapes:
    % 			Lucida Grande Mono 			ØOQ vs. default 0OQ;
    % 			Lucida Console 				ØOQ vs. default 0OQ.
    
    \setmainfont{LucidaBrightOT}[% main rm
          Ligatures=TeX,
          Extension=.otf,
          UprightFont=*,
          ItalicFont=*-Italic,
          BoldFont=*-Demi,
    	  BoldItalicFont=*-DemiItalic,
    %     BoldItalicFeatures={Color=Purple4}, % fixed 2024/10/13
    %     UprightFeatures={Color=Salmon3},
    	  Scale=0.93,% increased from 0.92, 2024/10/13
    %	  Numbers ={OldStyle}, 
      ]
    %
    \setsansfont{LucidaSansOT}[% main sans
          Ligatures=TeX,
          Extension=.otf,
          UprightFont=*,
          ItalicFont=*-Italic,
          BoldFont=*-Demi,
    	  BoldItalicFont=*-DemiItalic,
    	  Scale=MatchUppercase,
      ]
    %
    \setmonofont{LucidaSansTypewriterOT}[% main typewriter
          Ligatures=TeX,
          Extension=.otf,
          UprightFont=*,
          ItalicFont=*-Oblique,
          BoldFont=*-Bold,
          BoldItalicFont=*-BoldOblique,
          Scale=MatchLowercase,% changed from MatchUppercase, 2024/10/13
      ]
    
    %% MATH FONTS
    %
    % ss01 	alternate Latin lower case math italic identical to text italic. This option is not recommended as Greek 𝜈 (nu) and Latin 𝑣 (vee) become too similar
    % ss02 	smaller arrows (original Type 1 size): ⇑ vs. default ⇑.
    % ss03 	attempt to imitate Type 1 fonts
    % ss04 	calligraphic alternative (similar to the Type 1 design) to the math script alphabet
    % ss05 	use a slashed-zero style for the empty set character (U+2205): Ø vs. default ∅
    % ss08 	emphasize right and bottom edges of the d’Alembertian operator (U+29E0, \laplac), to follow the design of the Laplace operator (U+2206, \increment, Δ); the default design emphasizes the left and upper edges. Also available in the bold math font.
    %
    \setmathfont{LucidaBrightMathOT}[% main math
    	  Scale=MatchUppercase,
    	  Extension=.otf,
    	  BoldFont=LucidaBrightMathOT-Demi.otf,
%    	  BoldFeatures={Color=Chartreuse4},
    	  RawFeature ={+ss04,+ss08}, %
    ]
 
%% LucidaMath-OT contains a *serif* typerwriter font. If you prefer a sans serif typerwriter font, you can use the following two settings. 
% 
%    \setmathfont{LucidaSansTypewriterOT}[% <== NB: setting a text font where math font should go.
%    	  Scale=MatchUppercase,
%          range=tt,
%    	  Color=NavyBlue,
%          Extension=.otf,
%          script-features = {},     
%          sscript-features = {},     
%    	  BoldFont=LucidaSansTypewriterOT-Bold.otf,
%    	  BoldFeatures={Color=Salmon3},
%    ]
%    %
%    \setmathfontface\mathtt{LucidaSansTypewriterOT-Bold}[% bold upright typewriter font in boldmath.
%    	  version=bold,
%    	  Scale=MatchUppercase,
%          Extension=.otf,    
%    ]
	%
    \setmathfont{LucidaBrightMathOT}[%
    	  range={scr},% to make scr differ from cal
    	  RawFeature={-ss04},
    	  Scale=MatchUppercase,
          Extension=.otf,
    	  BoldFont=LucidaBrightMathOT-Demi.otf,% could be overridden by bold separate version
    ]
    \setmathfont{LucidaBrightMathOT}[% -Demi .. sufficient this way, since bold set above.
    	  range={bfscr},% need to call \symbfscr manually - bug in unicode-math version & range interaction
    	  RawFeature={-ss04},
    	  Scale=MatchUppercase,
          Extension=.otf,
    	  BoldFont=LucidaBrightMathOT-Demi.otf,
    ]
    %% Fix unicode-math operator font not set up for bold face (default \mathrm). See https://github.com/wspr/unicode-math/issues/468
    \setoperatorfont\normalfont
    %
    % note \mathbfit = \symbfit
    
    % The specialized one-off Lucida fonts:
    \newfontface\LucidaBlackletter{LucidaBlackletterOT}[%
    	Scale=0.95,% <== NB
    	Extension=.otf,
    	]
    \newfontface\LucidaCalligraphy{LucidaCalligraphyOT}[%
    	Scale=MatchUppercase,
    	Extension=.otf,
    	]
    \newfontface\LucidaHandwriting{LucidaHandwritingOT}[%
    	Scale=MatchUppercase,
    	Extension=.otf,
     	]
    % GrandeMono and Console fonts:
    \newfontface\LucidaGrandeMonoDK{LucidaGrandeMonoDK}[%	
    	Scale=MatchUppercase,
    	Extension=.otf,
        UprightFont=*,
        ItalicFont=*-Italic,
        BoldFont=*-Bold,
        BoldItalicFont=*-BoldItalic,
    	]
    \newfontface\LucidaConsole{LucidaConsoleDK}[%
    	Scale=MatchLowercase,% <=== NB
    	Extension=.otf,
        UprightFont=*,
        ItalicFont=*-Italic,
        BoldFont=*-Bold,
        BoldItalicFont=*-BoldItalic,
    	]
\fi


==> fontsets/mitthesis-newtx-sans-text.tex <==
% From mitthesis package
% Documentation: https://ctan.org/pkg/mitthesis

\ProvidesFile{mitthesis-newtx-sans-text.tex}[2024/06/68 v1.04 Load newtx sans-serif text and regular math fonts]

%% newtx package with sans-serif text (Helvetica-like text with Times-like math)
%
\ifpdftex
	\ClassNoteNoLine{\ClassName}{Loading newtx sans-serif text and newtx serif math fonts}
	\RequirePackage[T1]{fontenc}
    \RequirePackage[subscriptcorrection,varvw,helvratio=0.91,defaultsups]{newtx}% upint for upright integrals
	\AtEndPreamble{% added to accommodate v1.731 of newtx, 2023/11/03
	    \renewcommand{\familydefault}{\sfdefault}% use sans for main text
%	    \renewcommand{\rmdefault}{\sfdefault}% uses sans for \textrm{}, if that's desired.
	}
%   these two commands enable hyphenation of the typewriter font - https://tex.stackexchange.com/a/204421/119566
%    \input{t1ntxtt.fd}
%    \DeclareFontFamily{\encodingdefault}{\ttdefault}{\hyphenchar\font=`\-} % 
	\RequirePackage{bm}% bold math
\else
	\ClassWarning{\ClassName}{The newtx font set requires pdflatex.  Defaulting to LMR fonts}
    \RequirePackage[warnings-off={mathtools-colon,mathtools-overbracket}]{unicode-math}
    % suppress tiresome warnings about lack of integration between mathtools and unicode-math.
    % Unicode-math loads the fontspec package, but the default fonts are not selected by fontspec in this case.
\fi

	

==> fontsets/mitthesis-newtx.tex <==
% From mitthesis package
% Documentation: https://ctan.org/pkg/mitthesis

\ProvidesFile{mitthesis-newtx.tex}[2024/06/28 v1.04 Load newtx text and math fonts]

\ifpdftex
	\ClassNoteNoLine{\ClassName}{Loading newtx fonts with inconsolata typewriter}
	\RequirePackage[T1]{fontenc}
    \RequirePackage[subscriptcorrection,varvw,helvratio=0.91]{newtx}% stix2, upint
    \RequirePackage[varl,varqu,hyphenate,mono]{inconsolata}% sans typewriter font; mono = fixed word spacing, hyphenate = allow hyphenation 
	\RequirePackage{bm}
	\let\textsuperscript\textsu% newtx changes the default superiors font; this is needed to get commas aligned in sequential footnotes
\else
	\ClassWarning{\ClassName}{The newtx font set requires pdflatex.  Defaulting to LMR fonts}
    \RequirePackage[warnings-off={mathtools-colon,mathtools-overbracket}]{unicode-math}
    % suppress tiresome warnings about lack of integration between mathtools and unicode-math.
    % Unicode-math loads the fontspec package, but the default fonts are not selected by fontspec in this case.
\fi

	

==> fontsets/mitthesis-stix2.tex <==
% From mitthesis package
% Documentation: https://ctan.org/pkg/mitthesis

\ProvidesFile{mitthesis-stix2.tex}[2024/10/13 v1.06 Load STIX Two text and math fonts]

%% STIX Two text and math fonts with Heros sans serif font and Inconsolata monospaced font
%
% These fonts are available at: 
%				https://github.com/stipub/stixfonts 
%				http://www.gust.org.pl/projects/e-foundry/tex-gyre 
%				https://ctan.org/tex-archive/fonts/inconsolata
% Install these as system fonts on your computer
%
\ifpdftex
	\ClassError{\ClassName}{The stix2 fontset requires a unicode engine. Defaulting to CMR fonts.}{Use LuaLatex to run with the class option [fontset=stix2]}
	\RequirePackage[T1]{fontenc}	
	\RequirePackage{bm}
\else
	\ClassNoteNoLine{\ClassName}{Loading STIX Two text and math fonts with Heros sans serif font and Inconsolata monospaced font}
	%
    \RequirePackage[warnings-off={mathtools-colon,mathtools-overbracket}]{unicode-math}
    % suppress tiresome warnings about lack of integration between mathtools and unicode-math
    % unicode-math loads the fontspec package
	%
    \setmainfont{STIXTwoText}[% Presumes these are system fonts! 
       	Extension = .otf,
    	UprightFont = *-Regular,
    	ItalicFont = *-Italic,
    	BoldFont = *-Bold,
    	BoldItalicFont = *-BoldItalic,
		SlantedFont = *-Italic,
	]
	\setsansfont{texgyreheros}[% Presumes these are system fonts! 
		WordSpace = {1,1.4,1},
		Extension = .otf,
    	UprightFont = *-regular,
    	ItalicFont = *-italic,
    	BoldFont = *-bold,
    	BoldItalicFont = *-bolditalic,
		Numbers = Lining,
    	Scale=0.91,% 
	]        
	\setmonofont{Inconsolatazi4}[% This otf font ships with the LaTeX Inconsolata package (it's in TeX Live)
        Scale=1.035,% 2024/10/13
        Extension = .otf,
        UprightFont = *-Regular,
        ItalicFont = *-Regular,% has no italic face
        BoldFont = *-Bold, 
    	BoldItalicFont = *-Bold,% has no bold italic face
        RawFeature = {+ss01,+ss02,+ss03},
    ]             
	\setmathfont{STIXTwoMath-Regular}[% nice glyphs, but \mkern sometimes needed
    	Scale=MatchUppercase,
    	Extension = .otf,
%       Color=NavyBlue, 
    	RawFeature = {+ss01, -ss02, -ss08},
   ]
   % ss01 -- switch calligraphic to script; +ss02 -- variants of g, u, v, w, z; +ss08 -- upright integrals
   %
   \newcommand*{\FRAC}[1]{{\addfontfeature{Fractions=On}#1}}% use OpenType feature for fractions, \FRAC{1/2} 
\fi


==> fontsets/mitthesis-termes-stix2.tex <==
% From mitthesis package
% Documentation: https://ctan.org/pkg/mitthesis

\ProvidesFile{mitthesis-termes-stix2.tex}[2024/10/12 v1.06 Load TeX Gyre Termes text font with STIX2 math font, Heros sans serif font, and Inconsolata monospaced font]

%% TeX Gyre Termes text font and Heros sans serif font with STIX2 math font and Inconsolata monospaced font
%
% These fonts are available at: 
%				http://www.gust.org.pl/projects/e-foundry/tex-gyre 
%				https://github.com/stipub/stixfonts 
%				https://ctan.org/tex-archive/fonts/inconsolata
% Install these as system fonts on your computer
%
\ifpdftex
	\ClassError{\ClassName}{The termes-stix2 fontset requires a unicode engine. Defaulting to CMR fonts}{To use the class option [fontset=termes-stix2], use a unicode engine such as LuaLaTeX.}
	\RequirePackage[T1]{fontenc}	
	\RequirePackage{bm}
\else
	\ClassNoteNoLine{\ClassName}{Loading TeX Gyre Termes text font with STIX2 math font, Heros sans serif font, and Inconsolata monospaced font}
	%
    \RequirePackage[warnings-off={mathtools-colon,mathtools-overbracket}]{unicode-math}
    % suppress tiresome warnings about lack of integration between mathtools and unicode-math
    % unicode-math loads the fontspec package
	%
    \setmainfont{TeXGyreTermesX}[% Presumes these are system fonts! Available at: http://www.gust.org.pl/projects/e-foundry/tex-gyre
		WordSpace = {1,1.4,1},%% This stretch matches newtxtext a little better. 1.4
    	Extension = .otf,
    	UprightFont = *-Regular,
    	ItalicFont = *-Italic,
    	BoldFont = *-Bold,
    	BoldItalicFont = *-BoldItalic,
		SlantedFont = *-Italic,
		Numbers = Lining,
	]
	\setsansfont{texgyreheros}[% Presumes these are system fonts! Available at: http://www.gust.org.pl/projects/e-foundry/tex-gyre
		WordSpace = {1,1.4,1},
		Extension = .otf,
    	UprightFont = *-regular,
    	ItalicFont = *-italic,
    	BoldFont = *-bold,
    	BoldItalicFont = *-bolditalic,
		Numbers = Lining,
    	Scale=0.91,% same as for newtx; former value 0.9 too small 2022/01/15
	]        
	\setmonofont{Inconsolatazi4}[% This otf font ships with the LaTeX Inconsolata package (it's in TeX Live)
        Scale=1,% reset to 1, 2024/10/12 %1.03,% rescaled from 1, 22/03/10
        Extension = .otf,
        UprightFont = *-Regular,
        ItalicFont = *-Regular,% has no italic face
        BoldFont = *-Bold, 
    	BoldItalicFont = *-Bold,% has no bold italic face
        RawFeature = {+ss01,+ss02,+ss03},
    ]             
	\setmathfont{STIXTwoMath-Regular}[% nice glyphs, but \mkern sometimes needed %% https://github.com/stipub/stixfonts
    	Scale=MatchUppercase,
    	Extension = .otf,
%		BoldFont = *,% STIX Two Math has no bold face
%       Color=NavyBlue, 
    	RawFeature = {+ss01, -ss02, -ss08},
   ]
   % ss01 -- switch calligraphic to script; +ss02 -- variants of g, u, v, w, z; +ss08 -- upright integrals
   %
   \setmathfontface\mathbf{STIXTwoText-Bold.otf}[]% to not get Termes bold, https://github.com/stipub/stixfonts
   \setmathfontface\mathit{STIXTwoText-Italic.otf}[]
   \setmathfontface\mathrm{STIXTwoText-Regular.otf}[]% to get roman letters from STIX, not Termes
    %      
   \newcommand*{\FRAC}[1]{{\addfontfeature{Fractions=On}#1}}% use OpenType feature for fractions, \FRAC{1/2} 
\fi


==> fontsets/mitthesis-termes.tex <==
% From mitthesis package
% Documentation: https://ctan.org/pkg/mitthesis

\ProvidesFile{mitthesis-termes.tex}[2024/10/12 v1.05 Load TeX Gyre Termes text and math fonts, Heros sans serif font, and Cursor monospaced font]

%% TeX Gyre Termes (Times-like) text font with Termes math font and Heros sans serif font and Cursor monospaced font
%
% These fonts are available at: http://www.gust.org.pl/projects/e-foundry/tex-gyre
% install these as system fonts on your computer
%
\ifpdftex
	\ClassError{\ClassName}{The termes fontset requires a unicode engine. Defaulting to CMR fonts}{To use the class option [fontset=termes], use a unicode engine such as LuaLaTeX.}
	\RequirePackage[T1]{fontenc}	
	\RequirePackage{bm}
\else
	\ClassNoteNoLine{\ClassName}{Loading TeX Gyre Termes text and math fonts, Heros sans serif font, and Cursor monospaced font}
    \RequirePackage[warnings-off={mathtools-colon,mathtools-overbracket}]{unicode-math}
    % suppress tiresome warnings about lack of integration between mathtools and unicode-math
    % unicode-math loads the fontspec package
	%
    \setmainfont{TeXGyreTermesX}[% Presumes these are system fonts! Available at: http://www.gust.org.pl/projects/e-foundry/tex-gyre
		WordSpace = {1,1.4,1},
    	Extension = .otf,
    	UprightFont = *-Regular,
    	ItalicFont = *-Italic,
    	BoldFont = *-Bold,
    	BoldItalicFont = *-BoldItalic,
		SlantedFont = *-Italic,
		Numbers = Lining,
	]
    \setsansfont{texgyreheros}[% Presumes these are system fonts! Available at: http://www.gust.org.pl/projects/e-foundry/tex-gyre
		WordSpace = {1,1.4,1},
		Extension = .otf,
    	UprightFont = *-regular,
    	ItalicFont = *-italic,
    	BoldFont = *-bold,
    	BoldItalicFont = *-bolditalic,
		Numbers = Lining,
    	Scale=0.91,% same as used in newtx; former value 0.9 too small 2022/01/15
	]        
   \setmonofont{texgyrecursor}[% Presumes these are system fonts! Available at: http://www.gust.org.pl/projects/e-foundry/tex-gyre
        %Scale=0.97,
        Scale=1.03, % adjusted 2024/10/12 to bring x-size closer to other fonts
        Extension = .otf,
        UprightFont = *-Regular,
        ItalicFont = *-Italic,
        BoldFont = *-Bold, 
    	BoldItalicFont = *-BoldItalic,
%		BoldFeatures = { Color = VioletRed3 },
    ]             
    \setmathfont{texgyretermes-math}[% Presumes these are system fonts! Available at: http://www.gust.org.pl/projects/e-foundry/tex-gyre
    	Scale=MatchUppercase,
    	Extension = .otf,
%		BoldFont = *, % termes-math does not have a bold version
%       Color=Red3, 
    ]
    %   
    \newcommand*{\FRAC}[1]{{\addfontfeature{Fractions=On}#1}}% use OpenType feature for fractions, \FRAC{1/2}
\fi

